Node Weighted Scheduling

This paper proposes a new class of online policies for scheduling in input-buffered crossbar switches. Our policies are throughput optimal for a large class of arrival processes which satisfy strong-law of large numbers. Given an initial configuration and no further arrivals, our policies drain all packets in the system in the minimal amount of time (providing an online alternative to the batch approach based on Birkhoff-VonNeumann decompositions). We show that it is possible for policies in our class to be throughput optimal even if they are not constrained to be maximal in every time slot. Most algorithms for switch scheduling take an edge based approach; in contrast, we focus on scheduling (a large enough set of) the most congested ports. This alternate approach allows for lower-complexity algorithms, and also requires a non-standard technique to prove throughput-optimality. One algorithm in our class, Maximum Vertex-weighted Matching (MVM) has worst-case complexity similar to Max-size Matching, and in simulations shows slightly better delay performance than Max-(edge)weighted-Matching (MWM).

==> Extra.tex <==
The switch scheduling problem is to determine which matching is to be used in every time slot.


Most algorithms on switch scheduling take an edge based approach, attempting to schedule either a maximal/maximum set of edges, or those with the largest queues. In this paper we design policies that  look only at the weight of the \em{ports} in the switch; queues on the individual edges matter only to the extent that they are non-zero. Intuitively, our policies ensure scheduling of a large enough set of heavy ports in the system.





Our proof is based on the observation that all the ports that are critical (heaviest) in the fluid limit, may not remain heaviest in the neighborhood of time $t$, but they continue to be above a certain threshold. We show that the optimal threshold must be below this threshold and hence all the critical ports are scheduled in {em every} time-slot near to $t$.

Switch scheduling has been studied extensively both because of its relevance to high speed switching and its pedagogical example as a network complex enough to inspire interesting research yet simple enough for an extensive network theory to be developed.

The MWM algorithm for example is throughput optimal, not only for the switch network with cross bar constraints, but more general network like wireless networks with interference constraints.

Our node based policies, with weight of the node being equal to the sum of weights of the edges touching the nodes translates to the sum of weights of constraint sets like cliques in the general graph setting. It would be interesting to explore constraint weight based scheduling rules for these networks. For such a setting, a suitable Lyapunov function might be the heaviest constraint set.

Such a Lyapunov function has been used for the greedy maximal matching policy, where it has been established that GMM achieves full throughput if the underlying graph satisfies a local pooling condition. In contrast to the policy analyzed there, in our analysis, the LHPF policies need not even be maximal to guarantee throughput optimality.

The LHPF class of policies do not care about the weight of edges as far as the required nodes have been scheduled. This relieves a lot of computational overhead for the scheduler.


As noted in \cite{Mc98}, the MVM policy combines the benefit a maximum size algorithm, with those of a maximum weight algorithm, while lending itself to simple implementation in hardware. In MVM, each weight is a function of queue lengths (sum of all edges that touch a node) and hence has a advantage of both the maximum size matchings with high instantaneous throughput while guaranteeing high throughput, even when the arrival traffic is non-uniform.

The analysis is still limited to MWM type algorithms \cite{Sasha04, ShahWischik} because of the lack of any other Lyapunov function. The Lyapunov function designed here is much simpler, and opens avenues for the development of fluid analysis of such systems.


 Explanation of Figure 1.
 In Figure 1 shows the classes of online policies. The critical port policies are clearance time optimal but may not be throughput optimal in general. Among the class of critical port policies, we have established in this paper that LHPF policies are throughput optimal. MVM policy is a member of the class of LHPF policies and is also a member of the class of Maximum Size matchings. Note that there may be many maximum size matchings in a graph and different tie break rules will produce different matchings not all of which are throughput optimal. Finally this figure shows that MWM is throughput optimal but is not a critical port policy and hence is not clearance time optimal.


 Explanation of Figure 2

 Consider a 4$\times$4 switch with edge weights as shown in the figure. There is only one critical port (port a) with weight 10. So a critical port policy must at least schedule port a. Now let us consider a LHPF matching. Since there are only three ports with non-zero weights on the input side, the maximum size of a matching can at most be three. It follows that not all the ports on the output side can be matched, in particular





 This allows us to  {\em post-process}, i.e. make minimal changes to, schedules from any other algorithm, making it throughput-optimal.
